Learning Action Embeddings for Off-Policy Evaluation

Off-policy evaluation (OPE) methods allow us to compute the expected reward of a policy by using the logged data collected by a different policy. OPE is a viable alternative to running expensive online A/B tests: it can speed up the development of new policies, and reduces the risk of exposing customers to suboptimal treatments. However, when the number of actions is large, or certain actions are under-explored by the logging policy, existing estimators based on inverse-propensity scoring (IPS) can have a high or even infinite variance. Saito and Joachims (arXiv:2202.06317v2 [cs.LG]) propose marginalized IPS (MIPS) that uses action embeddings instead, which reduces the variance of IPS in large action spaces. MIPS assumes that good action embeddings can be defined by the practitioner, which is difficult to do in many real-world applications. In this work, we explore learning action embeddings from logged data. In particular, we use intermediate outputs of a trained reward model to define action embeddings for MIPS. This approach extends MIPS to more applications, and in our experiments improves upon MIPS with pre-defined embeddings, as well as standard baselines, both on synthetic and real-world data. Our method does not make assumptions about the reward model class, and supports using additional action information to further improve the estimates. The proposed approach presents an appealing alternative to DR for combining the low variance of DM with the low bias of IPS.

==> 00_outline.tex <==
\section*{Outline}

\emph{Introduction:} 
We want to evaluate the quality of recommender system policies, this is commonly done in a multi-armed bandit framework.
A standard way is to evaluate the policy online, but recently we aim to evaluate offline for many advantages.
Common estimators in off-policy evaluation have their disadvantages, namely increased variance due to the large action space.
Using pre-defined embeddings helps to reduce the variance for propensity based estimators.
Can we learn useful embeddings that improve the performance of MIPS?
Listed contributions.

\emph{Background and related work:}
Background pretty much the same as we had in the workshop paper.
Related work touching other relevant OPE methods: DM, DR, SNIPS and other additions, concluding there is nothing solving large action spaces without pre-defined embeddings.
Learning action representations in reinforcement learning: revisiting what we already wrote and clean this up.
Using the structure of the action space in multi-armed bandits: clean things up, here we touch multiple distinct fields - linear bandits, hierarchical bandits, combinatorial bandits, learning to rank, etc.

\emph{Dimensionality reduction effect on bias-variance trade-off:}
Here we make theoretical foundations for our approach, we can leverage other theoretical works \citep{yin2018dimensionality} how bias and variance are decomposed when using matrix factorization.
This is followed by our analysis connecting it to off-policy, showing how our bias-variance error is bounded by changing the number of dimensions.
We propose a basic linear neural network for extracting embeddings and state our hypothesis for deeper non-linear network to capture more complex functions.

\emph{Synthetic linear experiments:}
Experiments as in the original paper, but with hidden some dimensions to test if we can retrieve them and beat MIPS.

\emph{Synthetic neural network generated experiments:}
Experiments showing that when reward generating method is more complex, we may use more complex network to capture better embeddings.

\emph{Real-world dataset:}
Experiments showing the performance of all methods on real-world dataset.

\emph{Conclusions:}
Summarizing the results, findings and proposing future work (e.g. estimating embedding propensities using a prescribed form).

==> 0A_other_experiments.tex <==
\section{Additional Experiments}
\label{appendix: additional experiments}

In this section, we present additional experiments that further solidify the findings already discussed in \cref{sec: evaluation}. 
We show that learning the embeddings works even if the reward model cannot fit the reward-generating function well. 
Furthermore, we perform an ablation study where we show how varying the size of the learned embeddings impacts the bias-variance trade-off. 
Finally, we show additional results on the real-world data with increased sample size. 

\begin{figure*}[b]
    \centering
    \begin{subfigure}[t]{\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figs/nonlinear/legend.pdf}
    \end{subfigure}
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figs/nonlinear/nactions.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figs/nonlinear/nvaldata.pdf}
    \end{subfigure}
    \caption{Synthetic experiments with non-linear reward function. There are still substantial improvements with \emph{Learned MIPS OneHot} even when the reward model does not match the reward function. Fine-tuning embeddings with \emph{Learned MIPS FineTune} improves upon low-variance unbiased pre-defined embeddings when they are non-linear w.r.t.\ the reward.}
    \label{fig: synthetic nonlinear}
\end{figure*}


\paragraph{Can we get good estimates when the learned reward model can not capture the true reward function?}
The experiments conducted in the \cref{sec: evaluation} use the data generated from a reward function \eqref{eq: expected reward} that is linear w.r.t.\ context.
In this experiment, the reward function $q(x, e)$ is represented by a randomly initialized dense neural network with two non-linear hidden layers.
The neural network has an input in the form of a context vector concatenated with a one-hot encoded vector of the pre-defined categorical action embedding.
As in the other experiments, we use the same linear model for the DM and \emph{Learned MIPS OneHot}. 
The number of pre-defined embedding dimensions is fixed at $d_\cE = 3$.
Overall, the rest of the parameters is kept the same as in the first experiment in \cref{sec: synthetic experiments}.
\cref{fig: synthetic nonlinear} shows the similar results to \cref{fig: synthetic linear} and confirms our earlier findings.
Learning the action embeddings is still beneficial even when the reward model is misspecified, and Learned MIPS outperforms both DM and IPS.
This shows the robustness of this method against model misspecification.
Moreover, we hypothesize that when the reward is non-linear w.r.t\ pre-defined embeddings, we may benefit from fine-tuning pre-defined embeddings as we assume that logistic regression used to infer $p(a\mid e)$ learns the best propensities when the effect of individual features on the reward is independent of the others.
Unlike the low-variance, low-bias linear embeddings that were shown in \cref{fig: synthetic linear}, where we did not see any improvements by fine-tuning them, in \cref{fig: synthetic nonlinear} we can see substantial improvements when doing so.

\paragraph{How does the size of the learned embedding impact the bias and the variance of the estimate?}
In this experiment, we study whether we can explicitly control the bias-variance trade-off of the MIPS estimator when learning the embeddings by performing implicit matrix factorization.
We set the number of dimensions in the context vector at $d_\cX = 100$ and keep the rest of the parameters as in the first experiment in \cref{sec: synthetic experiments}. 
Instead of using a linear model, we define the training objective as a low-rank approximation.
We then vary the size of the learned embeddings to see whether there is any benefit in compressing the information into the smaller number of dimensions.
We sample the logged data 100 times for each setting and plot the relative MSE w.r.t\ IPS.
\cref{fig: ablation} shows us that for the sample size $n = 20000$, the optimal number of dimensions for learned embedding is about $8 - 16$. 
If the number of dimensions is too low, the added bias is higher than the amount of reduced variance. 
These results show there is a potential to further reduce variance of learned embeddings by optimizing for this parameter.

\paragraph{How does our method perform with increased sample size on real-world data?}
Here we show the performance of our method on the same real-world dataset as in \cref{sec: real world experiments}. 
We set the sample size at $n \in [50000, 100000]$ and keep the rest of the parameters fixed. 
\cref{fig: real-world extended} shows the cumulative distribution function of relative MSEs w.r.t.\ IPS.
DM is using the same underlying model as \emph{Learned MIPS OneHot} and similarly as in \cref{fig: real world data}, we see that even when the model fails to accurately predict the reward, it can still be used to derive useful embeddings for MIPS.
Additionally, we compare against two other competitive baselines, namely SNIPS \citep{swaminathan2015self} and Switch-DR \citep{wang2017optimal}, outperforming both of them.

\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.327\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figs/ablation/learned-embed-dim.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.667\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figs/ablation/learned-embed-dim_bias-variance.pdf}
    \end{subfigure}
    \caption{Synthetic experiments varying the size of learned embeddings. Relative MSE refers to the MSE of \emph{Learned MIPS} divided by the MSE of IPS. Shaded areas are standard errors.}
    \label{fig: ablation}
\end{figure*}

\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figs/real_dataset/legend.pdf}
    \end{subfigure}
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figs/real_dataset/50000_IPS.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figs/real_dataset/100000_IPS.pdf}
    \end{subfigure}
    \caption{CDF of relative MSEs with 50000 (left) and 100000 (right) samples. The intersection of a method with IPS tells us the proportion of experiments in which the method performs better than IPS.}
    \label{fig: real-world extended}
\end{figure*}

